FACESEC: A Fine-grained Robustness Evaluation Framework for Face Recognition Systems

We present FACESEC, a framework for fine-grained robustness evaluation of face recognition systems. FACESEC evaluation is performed along four dimensions of adversarial modeling: the nature of perturbation (e.g., pixel-level or face accessories), the attacker's system knowledge (about training data and learning architecture), goals (dodging or impersonation), and capability (tailored to individual inputs or across sets of these). We use FACESEC to study five face recognition systems in both closed-set and open-set settings, and to evaluate the state-of-the-art approach for defending against physically realizable attacks on these. We find that accurate knowledge of neural architecture is significantly more important than knowledge of the training data in black-box attacks. Moreover, we observe that open-set face recognition systems are more vulnerable than closed-set systems under different types of attacks. The efficacy of attacks for other threat model variations, however, appears highly dependent on both the nature of perturbation and the neural network architecture. For example, attacks that involve adversarial face masks are usually more potent, even against adversarially trained models, and the ArcFace architecture tends to be more robust than the others.

==> backup.tex <==
\subsection{Robustness against Realizable Attacks with Enhanced Transferability}

\begin{table}[]
\centering
\caption{Attack success rate of transferred dodging PGD attacks on closed-set face recognition models.}
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Target Model}} & \multicolumn{4}{c|}{\textbf{Source Model}}                                    \\ \cline{2-5} 
                                       & \multicolumn{2}{c|}{\textbf{Single}} & \multicolumn{2}{c|}{\textbf{Ensemble}} \\ \cline{2-5} 
                                       & \textbf{w/o mmt}   & \textbf{w/mmt}  & \textbf{w/o mmt}    & \textbf{w/mmt}   \\ \hline \hline
VGGFace                                & 0.08               & 0.16            & 0.43                & 0.51             \\ \hline
FaceNet                                & 0.42               & 0.52            & 0.73                & 0.83             \\ \hline
ArcFace18                              & 0.42               & 0.51            & 0.87                & 0.92             \\ \hline
ArcFace50                              & 0.35               & 0.55            & 0.86                & 0.90             \\ \hline
ArcFace101                             & 0.32               & 0.39            & 0.71                & 0.78             \\ \hline
\end{tabular}
}
\label{tab:enhance_pgd}
\end{table}

\begin{table}[]
\centering
\caption{Attack success rate of transferred dodging sticker attacks on closed-set face recognition models.}
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Target Model}} & \multicolumn{4}{c|}{\textbf{Source Model}}                                    \\ \cline{2-5} 
                                       & \multicolumn{2}{c|}{\textbf{Single}} & \multicolumn{2}{c|}{\textbf{Ensemble}} \\ \cline{2-5} 
                                       & \textbf{w/o mmt}   & \textbf{w/mmt}  & \textbf{w/o mmt}    & \textbf{w/mmt}   \\ \hline \hline
VGGFace                                & 0.02               & 0.07            & 0.02                & 0.04             \\ \hline
FaceNet                                & 0.02               & 0.01            & 0.03                & 0.04             \\ \hline
ArcFace18                              & 0.00               & 0.00            & 0.01                & 0.01             \\ \hline
ArcFace50                              & 0.00               & 0.00            & 0.00                & 0.00             \\ \hline
ArcFace101                             & 0.00               & 0.04            & 0.01                & 0.03
\\ \hline
\end{tabular}
}
\label{tab:enhance_sticker}
\end{table}

\begin{table}[]
\centering
\caption{Attack success rate of transferred dodging eyeglass attacks on closed-set face recognition models.}
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Target Model}} & \multicolumn{4}{c|}{\textbf{Source Model}}                                    \\ \cline{2-5} 
                                       & \multicolumn{2}{c|}{\textbf{Single}} & \multicolumn{2}{c|}{\textbf{Ensemble}} \\ \cline{2-5} 
                                       & \textbf{w/o mmt}   & \textbf{w/mmt}  & \textbf{w/o mmt}    & \textbf{w/mmt}   \\ \hline \hline
VGGFace                                & 0.17               & 0.22            & 0.26                & 0.28             \\ \hline
FaceNet                                & 0.08               & 0.09            & 0.14                & 0.16             \\ \hline
ArcFace18                              & 0.02               & 0.03            & 0.11                & 0.12             \\ \hline
ArcFace50                              & 0.05               & 0.05            & 0.10               & 0.12             \\ \hline
ArcFace101                             & 0.02               & 0.04            & 0.02                & 0.03             \\ \hline
\end{tabular}
}
\label{tab:enhance_eyeglass}
\end{table}

\begin{table}[]
\centering
\caption{Attack success rate of transferred dodging face mask attacks on closed-set face recognition models.}
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{3}{*}{\textbf{Target Model}} & \multicolumn{4}{c|}{\textbf{Source Model}}                                    \\ \cline{2-5} 
                                       & \multicolumn{2}{c|}{\textbf{Single}} & \multicolumn{2}{c|}{\textbf{Ensemble}} \\ \cline{2-5} 
                                       & \textbf{w/o mmt}   & \textbf{w/mmt}  & \textbf{w/o mmt}    & \textbf{w/mmt}   \\ \hline \hline
VGGFace                                & 0.18               & 0.26            & 0.20                & 0.32             \\ \hline
FaceNet                                & 0.26               & 0.38            & 0.43                & 0.42             \\ \hline
ArcFace18                              & 0.21               & 0.33            & 0.20                & 0.33             \\ \hline
ArcFace50                              & 0.28               & 0.34            & 0.37                & 0.36             \\ \hline
ArcFace101                             & 0.22               & 0.34            & 0.30                & 0.36             \\ \hline
\end{tabular}
}
\label{tab:enhance_facemask}
\end{table}
\liang{}{This subsection will be put in the appendix due to the page limitation.}
Next, we evaluate the robustness of face recognition systems under physically realizable attacks with enhanced transferability.
As shown in the experimental results above, face recognition models can exhibit $>$90\% robustness against some realizable adversarial examples transferred from a single-based source model trained using the same training set as the target model but with a different neural architecture. 
Two questions, therefore, naturally arise: 1) whether face recognition models still remain robustness to realizable attacks whose transferability is enhanced using the ensemble-based attacks and the momentum method described in Section~\ref{sec:methodology}, and 2) if so, which one contributes more to the enhancement.
We used the following steps to answer the questions above.
First, we constructed an ensemble-based source model for each target face recognition model.
The ensemble consisted of the other four models; each was trained using the same training set but different neural architectures.
We then performed white-box attacks on this ensemble, evaluated the robustness of the target model against the produced adversarial examples (with and without using momentum to producing these) and compared it to the robustness when a single-based source model is applied.  
Due to page limitations, we only present the results for dodging attacks on closed-set face recognition models and defer the other results to the Appendix.

The results are presented in Table \ref{tab:enhance_pgd}, \ref{tab:enhance_sticker}, \ref{tab:enhance_eyeglass}, and \ref{tab:enhance_facemask}.
Again, for the transferred attack from single models, we present the attack success rate in response to the source model that exhibits the highest transferability.
Our first observation is that \emph{both using an ensemble-based source model and the momentum method can improve the transferability of digital attack examples.
Specifically, the transferability of PGD attacks can be significantly improved by the former and moderately enhanced by the latter}.
For example, as shown in Table~\ref{tab:enhance_pgd} by solely using an ensemble-based source model instead of single models, the attack success rate of transferred PGD attacks on ArcFace18 is significantly improved by 43\%.
By contrast, using the momentum method alone increases the attack success rate by 9\%.
Moreover, the combination of the two contributes to a nearly 50\% improvement in the transferability, which indicates that closed-set face recognition models are fairly fragile to digital attack examples transferred from an ensemble source model.
Our second observation is that \emph{the transferability enhancement approaches widely used in digital attacks may or may not work for physically reliable attacks}.
Specifically, as shown in Table \ref{tab:enhance_sticker} and \ref{tab:enhance_eyeglass}, using either the ensemble-based or the momentum method has only a negligible improvement in the transferability of the sticker and eyeglass attacks.
By contrast, they lead to moderate improvement ($\sim$15\% as shown in Table~\ref{tab:enhance_facemask}) in face mask attacks.
\emph{This indicates that each attack method has its own characteristics; enhancement or augment approaches that work for one attack may not work for others.
Hence, it is critical to include different types of attack methods when evaluating face recognition models' robustness}.  

==> content/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Below we briefly describe some of the related literature on face recognition models, as well as adversarial example attacks on these.

%[deep face recognition]
Face recognition using deep neural networks (henceforth, deep face recognition) has lead to significant recent success.
A variety of approaches have been proposed to treat face recognition as conventional \emph{multi-class classification} problems by using the standard softmax loss function in the training phase~\cite{taigman2014deepface, sun2014deepb, sun2014deepb}.
More recent studies adopt ideas from \emph{metric learning} so as to maximize \emph{intra-class distance} and minimzie \emph{inter-class distance} under a chosen metric space.
To accomplish this goal, these approaches either use \emph{Euclidean distance based} loss functions such as the triplet loss~\cite{schroff2015facenet, parkhi2015deep} and the center loss~\cite{wen2016discriminative}, or \emph{Angular Margin based} loss functions such as the large margin softmax loss~\cite{liu2016large}, the angular softmax~\cite{liu2017sphereface}, and the additive angular margin loss~\cite{deng2019arcface}.     

%[attacks and defense on face recognition]
Recent studies have shown that deep neural networks are vulnerable to adversarial example attacks.
These attacks produce \emph{imperceptible} perturbations on images in the digital space to mislead classification~\cite{szegedy14intriguing, goodfellow15explaining, carlini2017towards} (henceforth, \emph{digital attacks}). 
While a number of attacks on face recognition fall into this category (e.g., by adding small $\ell_p$ bounded noise over the entire input~\cite{dong2019efficient} or perceptible and semantically meaningful perturbation on a restricted area of the input~\cite{qiu2019semanticadv}), of particular interest in this domain, are attacks in the physical world (henceforth, \emph{physical attacks}). 
For example, an attacker can fool a face recognition system by wearing an adversarial eyeglass frame~\cite{sharif2016accessorize}, or using a sophisticated light projection on his face~\cite{nguyen2020adversarial}.
In this paper, we focus on \emph{digital attacks that can be realized in the physical world}.

%[evaluation method]
A recent work by Yang et al.~\cite{yang2020delving} has the strongest conceptual connection to our work.
However, the proposed evaluation method only appeals to digital attacks, leaving robustness of face recognition systems against attacks in the physical world unanswered.  
